A comparative study of star formation processes in different environments

In this thesis we have identified two star formation sites for star formation in galaxies which differ widely in metal content. We conclude that `massive' star formation that occurs in a high density, high metallicity environment, like that encountered in circumnuclear star-forming regions, takes place in systems that comply to the definition of super stellar clusters and that are arranged in star forming complexes. These complexes have Halpha luminosities, and therefore masses of ionizing stars, that overlap at the lower end with those found in HII galaxies, which have a much lower metallicity. The fact that their ionization structure and the temperature of their ionizing radiation field are very similar, point to stellar clusters in these two environments which have the same equivalent effective temperature. This is contrary to what is expected from stellar evolution models which predict lower stellar effective temperatures in high metallicity regions.

==> tables/ratios-pap.tex <==
 \begin{longtable}{lc|ccc|cccc|ccc}
 \caption{Relative reddening corrected line intensities [$F(H\beta)$=$I(H\beta)$=10000]\label{ratiostot 1}} \\
 \hline
  &  & \multicolumn{3}{c|}{SDSS J1455} & \multicolumn{4}{c|}{SDSS J1509} & \multicolumn{3}{c}{SDSS J1528} \\
 \multicolumn{1}{c}{$\lambda$ ({\AA})} & f($\lambda$) & -EW  & $I(\lambda)$ &  $I(\lambda)^\dag$ & -EW  & $I(\lambda)$ &   $I(\lambda)^\dag$ &  $I(\lambda)^\ddag$ & -EW  & $I(\lambda)$ &  $I(\lambda)^\ddag$  \\
  & & (\AA) & & & (\AA) & &  &  & (\AA) & &  \\
 \hline
 \endfirsthead
 
 \multicolumn{ 12}{l}{\footnotesize Table~\ref{ratiostot 1} continued}
  \\
 \hline
  &  & \multicolumn{3}{c|}{SDSS J1455} & \multicolumn{4}{c|}{SDSS J1509} & \multicolumn{3}{c}{SDSS J1528} \\
 \multicolumn{1}{c}{$\lambda$ ({\AA})} & f($\lambda$) & -EW  & $I(\lambda)$ &  $I(\lambda)^\dag$ & -EW  & $I(\lambda)$ &  $I(\lambda)^\dag$ &  $I(\lambda)^\ddag$ & -EW  & $I(\lambda)$ &  $I(\lambda)^\ddag$  \\
  & & (\AA) & & & (\AA) & &  &  & (\AA) & &  \\
 \hline
 \endhead
 
 \hline\multicolumn{ 12}{r}{\footnotesize\sl continued on next page}
 \endfoot
 
 \hline
 \noalign {\noindent$^a$\,possibly blend with an unknown line; $^b$\,[O{\sc ii}]\,$\lambda\lambda$\,3726\,+\,3729; $^c$\,[Fe{\sc iii}]\,$\lambda\lambda$\,4986\,+\,4987; $^d$\,[O{\sc ii}]\,$\lambda\lambda$\,7318\,+\,7320; $^e$\,[O{\sc ii}]\,$\lambda\lambda$\,7330\,+\,7331. $^\dag$ from \citet{2006A&A...448..955I}; they gave $^\gimel$\,[S{\sc ii}]\,$\lambda\lambda$\,6717\,+\,6731 and $^\beth$\,[O{\sc ii}]\,$\lambda\lambda$\,7319\,+\,7330. $^\ddag$ from \citet{1992A&A...253..349P}.}
 \endlastfoot
 
 
 3727 [O{\sc ii}]$^b$        &   0.271   &   91.6 & 11154$\pm$164 & 10920$\pm$400 & 131.7 & 15318$\pm$182 &  20970$\pm$760 & 18620$\pm$1800 &  177.4 & 22882$\pm$294 & 22390$\pm$2160  \\
 3734 H13                    &   0.270   &    1.1 &   130$\pm$31  &   ---         &   3.5 &   278$\pm$56  &    ---         &   ---          &    2.8 &   295$\pm$56  &   ---  \\
 3750 H12                    &   0.266   &    1.8 &   204$\pm$48  &   270$\pm$70  &   2.1 &   203$\pm$48  &    300$\pm$80  &   ---          &    2.9 &   315$\pm$64  &   ---  \\
 3770 H11                    &   0.261   &    1.9 &   222$\pm$27  &   470$\pm$70  &   2.4 &   236$\pm$38  &    460$\pm$80  &   ---          &    5.0 &   510$\pm$53  &   ---  \\
 3798 H10                    &   0.254   &    3.7 &   407$\pm$39  &   520$\pm$80  &   4.7 &   410$\pm$60  &    480$\pm$90  &   ---          &    7.6 &   709$\pm$70  &   ---  \\
 3820 He{\sc i}              &   0.249   &    0.6 &    81$\pm$16  &   ---         &   0.6 &    66$\pm$15  &    ---         &   ---          &   ---  &     ---       &   ---  \\
 3835 H9                     &   0.246   &    5.0 &   574$\pm$68  &   750$\pm$70  &   6.3 &   537$\pm$59  &    710$\pm$90  &   ---          &    7.6 &   820$\pm$58  &   ---  \\
 3868 [Ne{\sc iii}]          &   0.238   &   37.1 &  4792$\pm$105 &  5230$\pm$200 &  32.5 &  3501$\pm$109 &   4120$\pm$180 &  3980$\pm$380  &   39.0 &  4717$\pm$180 & 5370$\pm$520  \\
 3889 He{\sc i}+H8           &   0.233   &   16.1 &  1816$\pm$99  &   ---         &  16.4 &  1622$\pm$81  &    ---         &   ---          &   21.1 &  2151$\pm$74  & ---  \\
 3968 [Ne{\sc iii}]+H7       &   0.216   &   27.6 &  2996$\pm$71  &   ---         &  20.6 &  2262$\pm$113 &    ---         &  2570$\pm$250  &   35.3 &  3231$\pm$143 & 3020$\pm$290  \\
 4026 [N{\sc ii}]+He{\sc i}  &   0.203   &    1.2 &   148$\pm$22  &   ---         &   1.4 &   157$\pm$19  &    ---         &   ---          &    1.9 &   208$\pm$55  & ---  \\
 4068 [S{\sc ii}]            &   0.195   &    1.2 &   158$\pm$11  &   ---         &   1.7 &   199$\pm$19  &    ---         &   ---          &    2.0 &   214$\pm$18  & ---  \\
 4102 H$\delta$              &   0.188   &   24.4 &  2580$\pm$57  &  2590$\pm$120 &  26.8 &  2420$\pm$61  &   2730$\pm$140 &  2820$\pm$270  &   41.6 &  2824$\pm$94  & 2820$\pm$270  \\
 4340 H$\gamma$              &   0.142   &   48.8 &  4562$\pm$70  &  4710$\pm$180 &  54.1 &  4395$\pm$76  &   4860$\pm$200 &  4680$\pm$450  &   62.4 &  4773$\pm$76  & 4790$\pm$460  \\
 4363 [O{\sc iii}]           &   0.138   &    9.8 &  1022$\pm$35  &   990$\pm$60  &   4.2 &   420$\pm$21  &    500$\pm$60  &   550$\pm$80   &    5.4 &   500$\pm$22  & ---  \\
 4471 He{\sc i}              &   0.106   &    4.1 &   380$\pm$23  &   ---         &   5.1 &   454$\pm$32  &    ---         &   ---          &    5.8 &   465$\pm$28  & ---  \\
 4658 [Fe{\sc iii}]          &   0.053   &    0.3 &    28$\pm$4   &   110$\pm$40  &   1.1 &   106$\pm$12  &    110$\pm$50  &   ---          &    1.6 &   125$\pm$17  & ---  \\
 4686 He{\sc ii}             &   0.045   &    0.8 &    75$\pm$9   &   ---         &  ---  &        ---    &    ---         &   ---          &   ---  &       ---     & ---  \\
 4713 [Ar{\sc iv}]+He{\sc i} &   0.038   &    2.7 &   223$\pm$17  &   ---         &  ---  &        ---    &    ---         &   ---          &    1.0 &    79$\pm$24  & ---  \\
 4740 [Ar{\sc iv}]           &   0.031   &    1.2 &   103$\pm$14  &   110$\pm$40  &  ---  &        ---    &    ---         &   ---          &   ---  &        ---    & ---  \\
 4861 H$\beta$               &   0.000   &  132.8 & 10000$\pm$67  & 10000$\pm$340 & 123.4 & 10000$\pm$74  &  10000$\pm$350 & 10000$\pm$960  &  171.4 & 10000$\pm$116 & 10000$\pm$960  \\
 4881 [Fe{\sc iii}]          &  -0.005   &    0.3 &    25$\pm$6   &   ---         &  ---  &       ---     &    ---         &   ---          &   ---  &        ---    & ---  \\
 4921 He{\sc i}              &  -0.014   &    1.3 &    96$\pm$11  &   ---         &   1.1 &    99$\pm$12  &    ---         &   ---          &    1.9 &   114$\pm$17  & ---  \\
 4959 [O{\sc iii}]           &  -0.024   &  254.3 & 20456$\pm$134 & 21040$\pm$680 & 190.7 & 16751$\pm$148 &  16610$\pm$560 & 16600$\pm$1600 &  256.2 & 16557$\pm$173 & 15850$\pm$1530  \\
 4986 [Fe{\sc iii}]$^c$      &  -0.030   &    0.9 &    71$\pm$18  &    90$\pm$40  &   1.3 &   114$\pm$16  &    140$\pm$40  &   ---          &    2.0 &   129$\pm$31  & ---  \\
 5007 [O{\sc iii}]           &  -0.035   &  782.2 & 61355$\pm$336 &   ---         & 571.3 & 49942$\pm$153 &    ---         & 50120$\pm$4840 &  764.2 & 48932$\pm$292 & 47860$\pm$4620  \\
 5015 He{\sc i}              &  -0.037   &    3.1 &   234$\pm$20  &   ---         &   2.9 &   249$\pm$26  &    ---         &   ---          &    5.4 &   324$\pm$32  & ---  \\
 5199 [N{\sc i}]             &  -0.078   &    0.7 &    48$\pm$10  &   ---         &   1.4 &   105$\pm$20  &    ---         &   ---          &   ---  &        ---    & ---  \\
 5270 [Fe{\sc iii}]$^a$      &  -0.094   &    0.4 &    26$\pm$5   &   ---         &  ---  &        ---    &    ---         &   ---          &   ---  &        ---    & ---  \\
 5755 [N{\sc ii}]            &  -0.188   &   ---  &       ---     &   ---         &  ---  &        ---    &    ---         &   ---          &   ---  &        ---    & ---  \\
 5876 He{\sc i}              &  -0.209   &   22.4 &  1140$\pm$35  &  1090$\pm$60  &  21.6 &  1268$\pm$59  &   1120$\pm$70  &  1230$\pm$120  &   28.5 &  1227$\pm$36  & ---  \\
 6300 [O{\sc i}]             &  -0.276   &    5.5 &   257$\pm$11  &   210$\pm$30  &   7.7 &   452$\pm$26  &    400$\pm$40  &   ---          &   11.3 &   438$\pm$18  & 1200$\pm$180  \\
 6312 [S{\sc iii}]           &  -0.278   &    3.6 &   160$\pm$6   &   150$\pm$30  &   2.8 &   164$\pm$9   &    160$\pm$40  &   ---          &    4.3 &   168$\pm$10  & ---  \\
 6364 [O{\sc i}]             &  -0.285   &    2.0 &    95$\pm$19  &   ---         &   2.6 &   146$\pm$19  &    ---         &   ---          &    3.8 &   145$\pm$12  & ---  \\
 6548 [N{\sc ii}]            &  -0.311   &    6.2 &   273$\pm$15  &   ---         &   9.6 &   541$\pm$28  &    ---         &   ---          &   19.4 &   721$\pm$45  & ---  \\
 6563 H$\alpha$              &  -0.313   &  646.8 & 27756$\pm$183 & 28190$\pm$980 & 522.6 & 27969$\pm$141 &  28570$\pm$1020& 28180$\pm$2720 &  823.2 & 28888$\pm$169 & 29510$\pm$2850  \\
 6584 [N{\sc ii}]            &  -0.316   &   18.2 &   792$\pm$19  &   750$\pm$50  &  25.4 &  1387$\pm$37  &   1370$\pm$70  &  1910$\pm$180  &   54.0 &  1959$\pm$43  & 1450$\pm$140  \\
 6678 He{\sc i}              &  -0.329   &    9.7 &   350$\pm$38  &   ---         &   7.2 &   392$\pm$15  &    ---         &   ---          &   10.3 &   350$\pm$10  & ---  \\
 6717 [S{\sc ii}]            &  -0.334   &   21.9 &  1000$\pm$26  &  1720$\pm$70$^\gimel$  &  35.8 &  1966$\pm$48 &  2880$\pm$110$^\gimel$  &  2140$\pm$210  &   57.1 &  1923$\pm$75 & 1320$\pm$200  \\
 6731 [S{\sc ii}]            &  -0.336   &   14.5 &   788$\pm$22  &   ---         &  27.1 &  1488$\pm$40  &    ---         &  1780$\pm$170  &   43.7 &  1422$\pm$58  & 1120$\pm$170  \\
 7065 He{\sc i}              &  -0.377   &    8.3 &   293$\pm$12  &   ---         &   6.0 &   302$\pm$19  &    ---         &   ---          &    9.6 &   297$\pm$17  & ---  \\
 7136 [Ar{\sc iii}]          &  -0.385   &   18.5 &   662$\pm$30  &   590$\pm$40  &  19.1 &   982$\pm$29  &   790$\pm$50   &  1200$\pm$120  &   19.1 &        ---    & ---  \\
 7281 He{\sc i}$^a$          &  -0.402   &    2.1 &    78$\pm$9   &   ---         &  ---  &        ---    &    ---         &   ---          &    2.0 &    60$\pm$5   & ---  \\
 7319 [O{\sc ii}]$^d$        &  -0.406   &    5.3 &   181$\pm$9   & 290$\pm$40$^\beth$ &   4.8 &   203$\pm$9 &   410$\pm$50$^\beth$ & ---         &   10.0 &   296$\pm$17 & ---  \\
 7330 [O{\sc ii}]$^e$        &  -0.407   &    4.1 &   142$\pm$8   &   ---         &   4.0 &   167$\pm$8   &    ---         &   ---          &    8.2 &   238$\pm$12  & ---  \\
 7751 [Ar{\sc iii}]          &  -0.451   &    4.7 &   154$\pm$9   &   ---         &   5.2 &   242$\pm$16  &    ---         &   ---          &    8.1 &   210$\pm$13  & ---  \\
 8446 O{\sc i}               &  -0.513   &    1.7 &    46$\pm$8   &   ---         &   1.6 &    68$\pm$10  &    ---         &   ---          &   ---  &        ---    & ---  \\
 8503 P16                    &  -0.518   &    2.6 &    59$\pm$10  &   ---         &  ---  &        ---    &    ---         &   ---          &   ---  &        ---    & ---  \\
 8546 P15                    &  -0.521   &   ---  &       ---     &   ---         &  ---  &        ---    &    ---         &   ---          &   ---  &        ---    & ---  \\
 8599 P14                    &  -0.525   &   ---  &       ---     &   ---         &   3.5 &   100$\pm$33  &    ---         &   ---          &    4.8 &    72$\pm$13  & ---  \\
 8665 P13                    &  -0.531   &    4.9 &   105$\pm$18  &   ---         &   4.0 &   118$\pm$42  &    ---         &   ---          &    5.7 &   102$\pm$15  & ---  \\
 8751 P12                    &  -0.537   &    7.9 &   147$\pm$17  &   ---         &   5.0 &   154$\pm$47  &    ---         &   ---          &   12.0 &   145$\pm$16  & ---  \\
 8865 P11                    &  -0.546   &    8.3 &   181$\pm$22  &   ---         &  11.4 &   297$\pm$65  &    ---         &   ---          &   24.5 &   199$\pm$43  & ---  \\
 9014 P10                    &  -0.557   &   11.4 &   269$\pm$32  &   ---         &  33.6 &   447$\pm$93  &    ---         &   ---          &   ---  &        ---    & ---  \\
 9069 [S{\sc iii}]           &  -0.561   &   50.8 &  1154$\pm$59  &   ---         &  82.1 &  2546$\pm$120 &    ---         &   ---          &   88.1 &  1688$\pm$127 & ---  \\
 9229 P9                     &  -0.572   &   33.0 &   400$\pm$50  &   ---         &  27.2 &   595$\pm$98  &    ---         &   ---          &   31.9 &   292$\pm$86  & ---  \\
 9532 [S{\sc iii}]           &  -0.592   &  140.1 &  3278$\pm$148 &   ---         & 176.3 &  5181$\pm$256 &    ---         &   ---          &  506.6 &  4049$\pm$289 & ---  \\
 9547 P8                     &  -0.593   &   21.7 &   455$\pm$69  &   ---         &  43.5 &   876$\pm$129 &    ---         &   ---          &   ---  &        ---    & ---  \\
\multicolumn{2}{l|}{I(H$\beta$)(erg\,seg$^{-1}$\,cm$^{-2}$)}    & \multicolumn{2}{c}{1.49\,$\times$\,10$^{-14}$}  &   & \multicolumn{2}{c}{1.35\,$\times$\,10$^{-14}$}  &   &   & \multicolumn{2}{c}{1.73\,$\times$\,10$^{-14}$}  & 
  \\
\multicolumn{2}{l|}{c(H$\beta$)}     & \multicolumn{2}{c}{ 0.13$\pm$0.01 }    &  0.05   & \multicolumn{2}{c}{ 0.07$\pm$0.01 }    & 0.08   &  0.05  & \multicolumn{2}{c}{ 0.04$\pm$0.01 }   & 0.15
  \\
 
 
 \end{longtable}


\setcounter{table}{4}


 \begin{longtable}{lc|cccc|ccc|cc}
 \caption{{\it (cont.)} Relative reddening corrected line intensities [$F(H\beta)$=$I(H\beta)$=10000] \label{ratiostot 2}} \\
 \hline
  &  & \multicolumn{4}{c|}{SDSS J1540} & \multicolumn{3}{c|}{SDSS J1616} & \multicolumn{1}{c}{SDSS J1657} \\
 \multicolumn{1}{c}{$\lambda$ ({\AA})} & f($\lambda$) & -EW  & $I(\lambda)$ &  $I(\lambda)^\dag$ &  $I(\lambda)^\S$ & -EW  & $I(\lambda)$ &  $I(\lambda)^\dag$  & -EW  & $I(\lambda)$ \\
  & & (\AA) & & &  &  (\AA) & &  &  (\AA) &  \\
 \hline
 \endfirsthead
 
 \multicolumn{ 11}{l}{\footnotesize Table~\ref{ratiostot 2} continued}
  \\
 \hline
  &  & \multicolumn{4}{c|}{SDSS J1540} & \multicolumn{3}{c|}{SDSS J1616} & \multicolumn{2}{c}{SDSS J1657} \\
 \multicolumn{1}{c}{$\lambda$ ({\AA})} & f($\lambda$) & -EW  & $I(\lambda)$ &  $I(\lambda)^\dag$ &  $I(\lambda)^\S$ & -EW  & $I(\lambda)$ &  $I(\lambda)^\dag$  & -EW  & $I(\lambda)$ \\
  & & (\AA) & & &  &  (\AA) & &  &  (\AA) &  \\
 \hline
 \endhead
 
 \hline\multicolumn{ 11}{r}{\footnotesize\sl continued on next page}
 \endfoot
 
 \hline
 \noalign {\noindent$^a$\,possibly blend with an unknown line; $^b$\,[O{\sc ii}]\,$\lambda\lambda$\,3726\,+\,3729; $^c$\,[Fe{\sc iii}]\,$\lambda\lambda$\,4986\,+\,4987; $^d$\,[O{\sc ii}]\,$\lambda\lambda$\,7318\,+\,7320; $^e$\,[O{\sc ii}]\,$\lambda\lambda$\,7330\,+\,7331. $^\dag$ from \citet{2006A&A...448..955I}; they gave $^\gimel$\,[S{\sc ii}]\,$\lambda\lambda$\,6717\,+\,6731 and $^\beth$\,[O{\sc ii}]\,$\lambda\lambda$\,7319\,+\,7330. $^\S$ from \citet{2004ApJS..153..429K}; they gave $^\varkappa$\,[O{\sc ii}]\,$\lambda\lambda$\,7319\,+\,7330.}
 \endlastfoot
 
 
 3727 [O{\sc ii}]$^b$       &   0.271   &  232.8 &  21793$\pm$256 &   ---         &   ---         &   33.5 &  8491$\pm$196 &   ---         &  120.1 & 18832$\pm$230  \\
 3734 H13                   &   0.270   &    2.6 &    272$\pm$48  &   ---         &   ---         &   ---  &       ---     &   ---         &   ---  &       ---      \\
 3750 H12                   &   0.266   &   ---  &       ---      &   ---         &   ---         &    1.8 &   377$\pm$101 &   ---         &    1.9 &   232$\pm$47   \\
 3770 H11                   &   0.261   &    2.7 &    314$\pm$61  &   ---         &   ---         &    1.5 &   357$\pm$113 &   ---         &    2.3 &   293$\pm$40   \\
 3798 H10                   &   0.254   &    4.8 &    581$\pm$93  &   760$\pm$90  &   810$\pm$280 &    2.1 &   447$\pm$92  &   ---         &    4.1 &   500$\pm$68   \\
 3820 He{\sc i}             &   0.249   &    1.5 &    166$\pm$23  &   ---         &   ---         &   ---  &       ---     &   ---         &   ---  &       ---      \\
 3835 H9                    &   0.246   &    6.2 &    678$\pm$85  &   920$\pm$90  &   940$\pm$260 &    3.1 &   638$\pm$90  &   790$\pm$110 &    7.1 &   780$\pm$93   \\
 3868 [Ne{\sc iii}]         &   0.238   &   15.2 &   2142$\pm$82  &  1860$\pm$90  &   ---         &   17.2 &  4105$\pm$166 &  5450$\pm$230 &   23.1 &  3262$\pm$132  \\
 3889 He{\sc i}+H8          &   0.233   &   11.6 &   1445$\pm$113 &   ---         &   ---         &    7.3 &  1591$\pm$112 &   ---         &   14.0 &  1826$\pm$95   \\
 3968 [Ne{\sc iii}]+H7      &   0.216   &   21.9 &   2309$\pm$144 &   ---         &   ---         &   11.7 &  2563$\pm$125 &   ---         &   22.4 &  2456$\pm$121  \\
 4026 [N{\sc ii}]+He{\sc i} &   0.203   &   20.6 &   2505$\pm$78  &   ---         &   ---         &    0.4 &    94$\pm$15  &   ---         &    1.1 &   155$\pm$16   \\
 4068 [S{\sc ii}]           &   0.195   &    1.7 &    231$\pm$18  &   ---         &   ---         &    0.5 &   108$\pm$10  &   ---         &    1.4 &   198$\pm$15   \\
 4102 H$\delta$             &   0.188   &   23.7 &   2589$\pm$63  &  2570$\pm$120 &  2590$\pm$130 &   13.3 &  2530$\pm$67  & 2800$\pm$150  &   20.9 &  2432$\pm$65   \\
 4340 H$\gamma$             &   0.142   &   44.2 &   4753$\pm$61  &  4670$\pm$170 &  4640$\pm$100 &   26.7 &  4597$\pm$89  & 5000$\pm$200  &   43.1 &  4417$\pm$97   \\
 4363 [O{\sc iii}]          &   0.138   &    4.5 &    291$\pm$17  &   220$\pm$40  &   220$\pm$50  &    4.5 &   851$\pm$26  &  980$\pm$80   &    4.5 &   524$\pm$24   \\
 4471 He{\sc i}             &   0.106   &    4.7 &    463$\pm$33  &   ---         &   ---         &    2.5 &   404$\pm$32  &   ---         &    4.2 &   443$\pm$33   \\
 4658 [Fe{\sc iii}]         &   0.053   &    0.7 &     78$\pm$14  &   ---         &   ---         &   ---  &       ---     &   ---         &    1.0 &   107$\pm$16   \\
 4686 He{\sc ii}            &   0.045   &   ---  &       ---      &   ---         &   ---         &    2.1 &   329$\pm$43  &   310$\pm$60  &    1.2 &   126$\pm$14   \\
 4713 [Ar{\sc iv}]+He{\sc i}&   0.038   &   ---  &       ---      &   ---         &   ---         &   ---  &       ---     &   ---         &   ---  &       ---      \\
 4740 [Ar{\sc iv}]          &   0.031   &   ---  &       ---      &   ---         &   ---         &    0.5 &    69$\pm$22  &   ---         &   ---  &       ---      \\
 4861 H$\beta$              &   0.000   &  122.4 & 10000$\pm$76   & 10000$\pm$340 & 10000$\pm$100 &   83.0 & 10000$\pm$96  & 10000$\pm$350 &  117.8 & 10000$\pm$79   \\
 4881 [Fe{\sc iii}]         &  -0.005   &   ---  &       ---      &   ---         &   ---         &   ---  &       ---     &   ---         &   ---  &       ---      \\
 4921 He{\sc i}             &  -0.014   &    1.2 &   109$\pm$15   &   ---         &   ---         &    0.9 &   116$\pm$13  &   ---         &    0.8 &    75$\pm$14   \\
 4959 [O{\sc iii}]          &  -0.024   &  114.4 & 10480$\pm$75   &  9920$\pm$340 &  9830$\pm$90  &  156.5 & 20492$\pm$147 & 20380$\pm$680 &  152.5 & 14333$\pm$127  \\
 4986 [Fe{\sc iii}]$^c$     &  -0.030   &    0.9 &    84$\pm$12   &   180$\pm$40  &   ---         &   ---  &       ---     &   ---         &    1.4 &   135$\pm$28   \\
 5007 [O{\sc iii}]          &  -0.035   &  348.3 & 30942$\pm$188  &   ---         & 29000$\pm$230 &  480.7 & 61516$\pm$371 &   ---         &  455.1 & 43082$\pm$240  \\
 5015 He{\sc i}             &  -0.037   &    2.7 &   235$\pm$16   &   ---         &   ---         &    1.8 &   225$\pm$26  &   ---         &    2.4 &   222$\pm$23   \\
 5199 [N{\sc i}]            &  -0.078   &    2.0 &   151$\pm$27   &   ---         &   ---         &   ---  &       ---     &   ---         &    2.0 &   157$\pm$26   \\
 5270 [Fe{\sc iii}]$^a$     &  -0.094   &   ---  &       ---      &   ---         &   ---         &   ---  &       ---     &   ---         &   ---  &       ---      \\
 5755 [N{\sc ii}]           &  -0.188   &   ---  &       ---      &   ---         &   ---         &   ---  &       ---     &   ---         &   ---  &       ---      \\
 5876 He{\sc i}             &  -0.209   &   19.2 &  1155$\pm$36   &  1090$\pm$60  &   ---         &   13.7 &  1063$\pm$75  &   970$\pm$60  &   18.9 &  1116$\pm$44   \\
 6300 [O{\sc i}]            &  -0.276   &    6.4 &   335$\pm$14   &   330$\pm$30  &   ---         &    1.7 &   104$\pm$18  &   170$\pm$40  &    8.1 &   438$\pm$16   \\
 6312 [S{\sc iii}]          &  -0.278   &    2.6 &   139$\pm$10   &   110$\pm$30  &   ---         &    3.2 &   186$\pm$11  &   200$\pm$40  &    3.7 &   201$\pm$9    \\
 6364 [O{\sc i}]            &  -0.285   &    2.3 &   122$\pm$17   &   ---         &   ---         &    0.9 &    51$\pm$13  &   ---         &    2.8 &   152$\pm$18   \\
 6548 [N{\sc ii}]           &  -0.311   &   13.9 &   735$\pm$34   &   ---         &   ---         &    2.8 &   160$\pm$13  &   ---         &    9.4 &   464$\pm$23   \\
 6563 H$\alpha$             &  -0.313   &  581.9 & 28626$\pm$162  & 28770$\pm$1010& 28730$\pm$220 &  517.2 & 27892$\pm$145 & 28160$\pm$1000&  571.3 & 27772$\pm$153  \\
 6584 [N{\sc ii}]           &  -0.316   &   42.2 &  2116$\pm$66   &  1960$\pm$90  &   ---         &    8.0 &   434$\pm$23  &   380$\pm$40  &   28.8 &  1428$\pm$47   \\
 6678 He{\sc i}             &  -0.329   &    6.8 &   316$\pm$15   &   ---         &   ---         &    5.9 &   296$\pm$18  &   ---         &    6.7 &   315$\pm$18   \\
 6717 [S{\sc ii}]           &  -0.334   &   52.6 &  2609$\pm$52   &  4330$\pm$130$^\gimel$ & 2450$\pm$30 &   15.3 &   774$\pm$23  &  1400$\pm$70$^\gimel$  &   47.4 &  2207$\pm$57  \\
 6731 [S{\sc ii}]           &  -0.336   &   41.7 &  1919$\pm$50   &   ---         &  1800$\pm$30  &   11.9 &   581$\pm$22  &   ---         &   32.2 &  1598$\pm$43   \\
 7065 He{\sc i}             &  -0.377   &    4.5 &   200$\pm$9    &   ---         &   ---         &    5.1 &   229$\pm$14  &   ---         &    5.6 &   235$\pm$10   \\
 7136 [Ar{\sc iii}]         &  -0.385   &   23.2 &   892$\pm$52   &   880$\pm$50  &   ---         &   17.4 &   736$\pm$44  &   690$\pm$50  &   16.4 &   717$\pm$26   \\
 7281 He{\sc i}$^a$         &  -0.402   &    3.1 &   115$\pm$10   &   ---         &   ---         &   ---  &       ---     &   ---         &    0.9 &    41$\pm$7    \\
 7319 [O{\sc ii}]$^d$       &  -0.406   &    6.3 &   273$\pm$16   &   500$\pm$40$^\beth$  &  460$\pm$40$^\varkappa$ &    3.4 &   138$\pm$11  &  260$\pm$40$^\beth$  &   12.3 &   302$\pm$17  \\
 7330 [O{\sc ii}]$^e$       &  -0.407   &    5.0 &   216$\pm$12   &   ---         &   ---         &    2.2 &    90$\pm$7   &   ---         &    8.8 &   211$\pm$14   \\
 7751 [Ar{\sc iii}]         &  -0.451   &    6.1 &   223$\pm$26   &   ---         &   ---         &    4.5 &   166$\pm$21  &   ---         &    4.6 &   177$\pm$22   \\
 8446 O{\sc i}              &  -0.513   &   ---  &       ---      &   ---         &   ---         &   ---  &       ---     &   ---         &   ---  &       ---      \\
 8503 P16                   &  -0.518   &   ---  &       ---      &   ---         &   ---         &    2.6 &    60$\pm$20  &   ---         &   ---  &       ---      \\
 8546 P15                   &  -0.521   &   ---  &       ---      &   ---         &   ---         &    1.6 &    38$\pm$14  &   ---         &   ---  &       ---      \\
 8599 P14                   &  -0.525   &   ---  &       ---      &   ---         &   ---         &    5.6 &   109$\pm$20  &   ---         &   ---  &       ---      \\
 8665 P13                   &  -0.531   &   ---  &       ---      &   ---         &   ---         &    8.0 &   153$\pm$31  &   ---         &    7.7 &   144$\pm$53   \\
 8751 P12                   &  -0.537   &   ---  &       ---      &   ---         &   ---         &    8.1 &   181$\pm$32  &   ---         &    4.2 &   101$\pm$29   \\
 8865 P11                   &  -0.546   &   ---  &       ---      &   ---         &   ---         &    9.6 &   182$\pm$34  &   ---         &    8.5 &   211$\pm$34   \\
 9014 P10                   &  -0.557   &   12.9 &   237$\pm$68   &   ---         &   ---         &   24.4 &   319$\pm$44  &   ---         &   15.4 &   167$\pm$36   \\
 9069 [S{\sc iii}]          &  -0.561   &   67.2 &  2095$\pm$62   &  2020$\pm$100 &   ---         &   74.3 &  1647$\pm$62  &  1470$\pm$80  &   59.2 &  1400$\pm$99   \\
 9229 P9                    &  -0.572   &   ---  &       ---      &   ---         &   ---         &   14.2 &   272$\pm$51  &   ---         &   16.9 &   263$\pm$47   \\
 9532 [S{\sc iii}]          &  -0.592   &  236.8 &  5331$\pm$331  &   ---         &   ---         &   74.3 &  4011$\pm$153 &   ---         &  157.3 &  3674$\pm$257  \\
 9547 P8                    &  -0.593   &   29.0 &   573$\pm$145  &   ---         &   ---         &   ---  &       ---     &   ---         &   ---  &       ---      \\
I(H$\beta$)(erg\,seg$^{-1}$\,cm$^{-2}$) &   & \multicolumn{2}{c}{0.53\,$\times$\,10$^{-14}$}  &   &   & \multicolumn{2}{c}{1.36\,$\times$\,10$^{-14}$}  &  & \multicolumn{2}{c}{0.63\,$\times$\,10$^{-14}$}
  \\
c(H$\beta$) &     & \multicolumn{2}{c}{0.22$\pm$0.01}    & 0.07   &  0.07  & \multicolumn{2}{c}{0.02$\pm$0.01}     & 0.06  & \multicolumn{2}{c}{0.05$\pm$0.01}
  \\
 
 
 \end{longtable}


\setcounter{table}{4}


 \begin{longtable}{lc|cccc}
 \caption{{\it (cont.)} Relative reddening corrected line intensities [$F(H\beta)$=$I(H\beta)$=10000] \label{ratiostot 3}} \\
 \hline
  &  & \multicolumn{4}{c}{SDSS J1729} \\
 \multicolumn{1}{c}{$\lambda$ ({\AA})} & f($\lambda$) & -EW  & $I(\lambda)$ & $I(\lambda)^\dag$ &  $I(\lambda)^\S$ \\
  & & (\AA) &  \\
 \hline
 \endfirsthead
 
 \multicolumn{6}{l}{\footnotesize Table~\ref{ratiostot 3} continued}
  \\
 \hline
  &  & \multicolumn{4}{c}{SDSS J1729} \\
 \multicolumn{1}{c}{$\lambda$ ({\AA})} & f($\lambda$) & -EW  & $I(\lambda)$ & $I(\lambda)^\dag$ &  $I(\lambda)^\S$ \\
  & & (\AA) &  \\
 \hline
 \endhead
 
 \hline\multicolumn{6}{r}{\footnotesize\sl continued on next page}
 \endfoot
 
 \hline
 \noalign {\noindent$^a$\,possibly blend with an unknown line; $^b$\,[O{\sc ii}]\,$\lambda\lambda$\,3726\,+\,3729; $^c$\,[Fe{\sc iii}]\,$\lambda\lambda$\,4986\,+\,4987; $^d$\,[O{\sc ii}]\,$\lambda\lambda$\,7318\,+\,7320; $^e$\,[O{\sc ii}]\,$\lambda\lambda$\,7330\,+\,7331. $^\dag$ from \citet{2006A&A...448..955I}; they gave $^\gimel$\,[S{\sc ii}]\,$\lambda\lambda$\,6717\,+\,6731 and $^\beth$\,[O{\sc ii}]\,$\lambda\lambda$\,7319\,+\,7330. $^\S$ from \citet{2004ApJS..153..429K}; they gave $^\varkappa$\,[O{\sc ii}]\,$\lambda\lambda$\,7319\,+\,7330.}
 \endlastfoot
 
 
 3727 [O{\sc ii}]$^b$       &   0.271   &  135.8 & 17622$\pm$243 &   ---         & --- \\
 3734 H13                   &   0.270   &    1.4 &   175$\pm$54  &   ---         & --- \\
 3750 H12                   &   0.266   &    4.2 &   397$\pm$89  &   370$\pm$70  & --- \\
 3770 H11                   &   0.261   &    7.6 &   713$\pm$88  &   480$\pm$70  & --- \\
 3798 H10                   &   0.254   &    5.2 &   598$\pm$71  &   620$\pm$60  &   370$\pm$200 \\
 3820 He{\sc i}             &   0.249   &   ---  &       ---     &   ---         & --- \\
 3835 H9                    &   0.246   &    7.6 &   721$\pm$64  &   900$\pm$60  &   640$\pm$140 \\
 3868 [Ne{\sc iii}]         &   0.238   &   34.9 &  4787$\pm$172 &  3730$\pm$140 & --- \\
 3889 He{\sc i}+H8          &   0.233   &   16.9 &  2058$\pm$83  &   ---         & --- \\
 3968 [Ne{\sc iii}]+H7      &   0.216   &   24.7 &  2969$\pm$129 &   ---         & --- \\
 4026 [N{\sc ii}]+He{\sc i} &   0.203   &    2.4 &   311$\pm$30  &   ---         & --- \\
 4068 [S{\sc ii}]           &   0.195   &    0.9 &   122$\pm$11  &   ---         & --- \\
 4102 H$\delta$             &   0.188   &   24.9 &  2765$\pm$63  &  2540$\pm$100 &  2430$\pm$100 \\
 4340 H$\gamma$             &   0.142   &   48.7 &  4839$\pm$84  &  4760$\pm$170 &  4750$\pm$80  \\
 4363 [O{\sc iii}]          &   0.138   &    5.9 &   660$\pm$30  &   510$\pm$40  &   510$\pm$40  \\
 4471 He{\sc i}             &   0.106   &    5.2 &   516$\pm$24  &   ---         &   --- \\
 4658 [Fe{\sc iii}]         &   0.053   &    0.8 &    90$\pm$14  &   ---         &   --- \\
 4686 He{\sc ii}            &   0.045   &   ---  &      ---      &   ---         &   --- \\
 4713 [Ar{\sc iv}]+He{\sc i}&   0.038   &    0.7 &    77$\pm$16  &   ---         &   --- \\
 4740 [Ar{\sc iv}]          &   0.031   &    0.4 &    40$\pm$10  &   ---         &   --- \\
 4861 H$\beta$              &   0.000   &  125.6 & 10000$\pm$83  & 10000$\pm$320 & 10000$\pm$80  \\
 4881 [Fe{\sc iii}]         &  -0.005   &   ---  &      ---      &   ---         &   --- \\
 4921 He{\sc i}             &  -0.014   &    1.4 &   122$\pm$12  &   ---         &   --- \\
 4959 [O{\sc iii}]          &  -0.024   &  185.8 & 17097$\pm$146 & 16990$\pm$540 & 17470$\pm$90  \\
 4986 [Fe{\sc iii}]$^c$     &  -0.030   &    0.6 &    56$\pm$18  &    80$\pm$30  &  --- \\
 5007 [O{\sc iii}]          &  -0.035   &  555.4 & 51541$\pm$418 &   ---         & 52320$\pm$300 \\
 5015 He{\sc i}             &  -0.037   &    1.9 &   177$\pm$12  &   ---         &   --- \\
 5199 [N{\sc i}]            &  -0.078   &   ---  &      ---      &   ---         &   --- \\
 5270 [Fe{\sc iii}]$^a$     &  -0.094   &    0.7 &    55$\pm$12  &   ---         &   --- \\
 5755 [N{\sc ii}]           &  -0.188   &    0.8 &    60$\pm$6   &   ---         &   --- \\
 5876 He{\sc i}             &  -0.209   &   17.4 &  1261$\pm$37  &  1130$\pm$50  &   --- \\
 6300 [O{\sc i}]            &  -0.276   &    4.0 &   253$\pm$16  &   260$\pm$30  &   --- \\
 6312 [S{\sc iii}]          &  -0.278   &    2.7 &   176$\pm$11  &   170$\pm$30  &   --- \\
 6364 [O{\sc i}]            &  -0.285   &    1.2 &    78$\pm$11  &   ---         &   --- \\
 6548 [N{\sc ii}]           &  -0.311   &   12.5 &   771$\pm$21  &   ---         &   --- \\
 6563 H$\alpha$             &  -0.313   &  476.9 & 28700$\pm$163 & 28510$\pm$960 & 28530$\pm$150 \\
 6584 [N{\sc ii}]           &  -0.316   &   35.8 &  2189$\pm$52  &  2080$\pm$80  &   --- \\
 6678 He{\sc i}             &  -0.329   &    6.0 &   355$\pm$12  &   ---         &   --- \\
 6717 [S{\sc ii}]           &  -0.334   &   21.7 &  1286$\pm$32  &  2160$\pm$80$^\gimel$  & 1220$\pm$20 \\
 6731 [S{\sc ii}]           &  -0.336   &   17.3 &  1009$\pm$30  &   ---         & 950$\pm$20 \\
 7065 He{\sc i}             &  -0.377   &    5.7 &   265$\pm$18  &   ---         &   --- \\
 7136 [Ar{\sc iii}]         &  -0.385   &   18.0 &   864$\pm$41  &   950$\pm$50  &   --- \\
 7281 He{\sc i}$^a$         &  -0.402   &    1.5 &    75$\pm$11  &   ---         &   --- \\
 7319 [O{\sc ii}]$^d$       &  -0.406   &    4.6 &   233$\pm$8   &   430$\pm$40$^\beth$  & 390$\pm$20$^\varkappa$ \\
 7330 [O{\sc ii}]$^e$       &  -0.407   &    3.9 &   194$\pm$9   &   ---         &   --- \\
 7751 [Ar{\sc iii}]         &  -0.451   &    4.5 &   210$\pm$10  &   ---         &   --- \\
 8446 O{\sc i}              &  -0.513   &   ---  &      ---      &   ---         &   --- \\
 8503 P16                   &  -0.518   &    3.0 &   102$\pm$32  &   ---         &   --- \\
 8546 P15                   &  -0.521   &   ---  &      ---      &   ---         &   --- \\
 8599 P14                   &  -0.525   &    2.9 &    96$\pm$17  &   ---         &   --- \\
 8665 P13                   &  -0.531   &    4.7 &   140$\pm$20  &   ---         &   --- \\
 8751 P12                   &  -0.537   &    7.0 &   205$\pm$35  &   ---         &   --- \\
 8865 P11                   &  -0.546   &   ---  &      ---      &   ---         &   --- \\
 9014 P10                   &  -0.557   &    8.1 &   236$\pm$54  &   ---         &   --- \\
 9069 [S{\sc iii}]          &  -0.561   &   58.5 &  2092$\pm$95  &   ---         &   --- \\
 9229 P9                    &  -0.572   &   19.9 &   400$\pm$64  &   ---         &   --- \\
 9532 [S{\sc iii}]          &  -0.592   &  181.5 &  4718$\pm$250 &   ---         &   --- \\
 9547 P8                    &  -0.593   &   20.3 &   480$\pm$69  &   ---         &   --- \\
     I(H$\beta$)(erg\,seg$^{-1}$\,cm$^{-2}$) &   & \multicolumn{2}{c}{2.40\,$\times$\,10$^{-14}$} \\
     c(H$\beta$) &     & \multicolumn{2}{c}{0.03$\pm$0.01}     & 0.02   & 0.04  \\
 
 
 \end{longtable}




==> tables/temden-pap.tex <==
 \begin{table*}
 {\small
 \caption{Electron densities and temperatures for the observed CAHA galaxies.}
 \label{temden}
 \begin{center}
 \begin{tabular}{lcccccc}
 \hline
  & n([S{\sc ii}]) & t$_e$([O{\sc iii}]) &  t$_e$([O{\sc ii}]) & t$_e$([S{\sc iii}]) & t$_e$([S{\sc ii}]) &  t$_e$([N{\sc ii}])
  \\
 \hline
 
 
SDSS J1455                &  94 $\pm$ 40 & 1.40 $\pm$ 0.02 & 1.33 $\pm$ 0.07 & 1.37 $\pm$ 0.05 & 1.31 $\pm$ 0.11 &       ---       \\
SDSS J1509                &  85 $\pm$ 45 & 1.09 $\pm$ 0.01 & 1.18 $\pm$ 0.05 & 1.02 $\pm$ 0.04 & 0.89 $\pm$ 0.07 &       ---       \\
SDSS J1528                &  60:         & 1.16 $\pm$ 0.01 & 1.17 $\pm$ 0.05 & 1.21 $\pm$ 0.06 & 0.99 $\pm$ 0.07 &       ---       \\
SDSS J1540                &  47 $\pm$ 38 & 1.13 $\pm$ 0.02 & 1.15 $\pm$ 0.06 & 0.97 $\pm$ 0.04 & 0.85 $\pm$ 0.05 &       ---       \\
SDSS J1616                &  54:         & 1.30 $\pm$ 0.01 & 1.29 $\pm$ 0.09 & 1.29 $\pm$ 0.06 & 1.21 $\pm$ 0.12 &       ---       \\
SDSS J1657                &  30:         & 1.23 $\pm$ 0.02 & 1.33 $\pm$ 0.07 & 1.45 $\pm$ 0.08 & 0.88 $\pm$ 0.05 &       ---       \\
SDSS J1729                & 109 $\pm$ 47 & 1.26 $\pm$ 0.02 & 1.16 $\pm$ 0.04 & 1.13 $\pm$ 0.05 & 0.82 $\pm$ 0.06 & 1.40 $\pm$ 0.09 \\
 
 
 \hline
 \multicolumn{7}{l}{densities in $cm^{-3}$                 and temperatures in 10$^4$\,K}
 \end{tabular}
 \end{center}}
 \end{table*}

